Asymmetric cloning in quantum information theory

This thesis investigates quantum cloning and related quantum entanglement problems using core concepts of representation theory, in particular those associated with the symmetric group. The research explores Schur-Weyl duality and its extensions, which allow efficient representation and manipulation of quantum systems, serving as a valuable tool for quantum information theory. A primary application of Schur-Weyl duality is the quantum cloning problem, which is studied for both the $1 \to 2$ and the more general $1 \to N$ cases, providing new insights into the constraints imposed by the no-cloning theorem. The investigation extends to a more general quantum entanglement problem on a complete graph.

==> chapters/abstract.tex <==
\thispagestyle{empty}

\selectlanguage{french}
\noindent\textbf{Résumé :}\\
\par
Cette thèse étudie le clonage quantique et des problèmes relatifs d'intrication quantique en utilisant les concepts fondamentaux de la théorie des représentations, en particulier ceux associés au groupe symétrique. La recherche explore la dualité de Schur-Weyl et ses extensions, qui permettent une représentation et une manipulation efficaces des systèmes quantiques, constituant un outil précieux pour la théorie de l'information quantique.

Une application principale de la dualité de Schur-Weyl est le problème du clonage quantique, qui est étudié à la fois pour les cas 1 → 2 et pour les cas plus généraux 1 → N, apportant de nouvelles perspectives sur les contraintes imposées par le théorème du non-clonage. L'étude s'étend ensuite à un problème d'intrication quantique plus général sur un graphe complet.

La thèse est organisée en chapitres sur la dualité de Schur-Weyl, les fondations mathématiques de la mécanique quantique, les problèmes de clonage quantique et les problèmes d'intrication quantique, avec une annexe fournissant un aperçu de la théorie des représentations.

\vfill

\selectlanguage{english}
\noindent\textbf{Abstract:}\\
\par
This thesis investigates quantum cloning and related quantum entanglement problems using core concepts of representation theory, in particular those associated with the symmetric group. The research explores Schur-Weyl duality and its extensions, which allow efficient representation and manipulation of quantum systems, serving as a valuable tool for quantum information theory.

A primary application of Schur-Weyl duality is the quantum cloning problem, which is studied for both the 1 → 2 and the more general 1 → N cases, providing new insights into the constraints imposed by the no-cloning theorem. The investigation extends to a more general quantum entanglement problem on a complete graph.

The thesis is organized into chapters on Schur-Weyl duality, mathematical foundations of quantum mechanics, quantum cloning problems, and quantum entanglement problems, with an appendix providing an overview of representation theory.
